A Study of Situational Reasoning for Traffic Understanding

Intelligent Traffic Monitoring (ITMo) technologies hold the potential for improving road safety/security and for enabling smart city infrastructure. Understanding traffic situations requires a complex fusion of perceptual information with domain-specific and causal commonsense knowledge. Whereas prior work has provided benchmarks and methods for traffic monitoring, it remains unclear whether models can effectively align these information sources and reason in novel scenarios. To address this assessment gap, we devise three novel text-based tasks for situational reasoning in the traffic domain: i) BDD-QA, which evaluates the ability of Language Models (LMs) to perform situational decision-making, ii) TV-QA, which assesses LMs' abilities to reason about complex event causality, and iii) HDT-QA, which evaluates the ability of models to solve human driving exams. We adopt four knowledge-enhanced methods that have shown generalization capability across language reasoning tasks in prior work, based on natural language inference, commonsense knowledge-graph self-supervision, multi-QA joint training, and dense retrieval of domain information. We associate each method with a relevant knowledge source, including knowledge graphs, relevant benchmarks, and driving manuals. In extensive experiments, we benchmark various knowledge-aware methods against the three datasets, under zero-shot evaluation; we provide in-depth analyses of model performance on data partitions and examine model predictions categorically, to yield useful insights on traffic understanding, given different background knowledge and reasoning strategies.

==> sections/oldresult.tex <==

\section{Results}
\label{sec:result}

\subsection{Overall performance}

Table~\ref{tab: all result} shows the results for four different types of models (NLI-based, KG-based, and Multi-QA-based) on three datasets(BDD-QA, TV-QA, HDT-QA), together with random baseline, supervised and unsupervised model and human evaluation.

\para{BDD-QA} The T5-large model with an Information-Retrieval-Based approach yields the highest unsupervised accuracy among models with similar sizes, showing the benefit of the retrieved domain knowledge. However, this performance is only 0.287 points better than the random baseline and remains significantly behind the supervised model (0.357 points). Among the three commonly used knowledge zero-shot models (NLI, KG, QA), the KG-based models demonstrate lower performance compared to the NLI-based and QA-based models, indicating that general knowledge has a limited impact on decision-making in the traffic domain compared to semantic coherence and multi-QA training. The supervised training model has the highest accuracy across all action classes with scores ranging from 0.774 to 0.968. This is intuitive because the domain in BDD-QA is narrower than other typical QA models, the environment and the corresponding actions are easy to capture as a result. 

\para{TV-QA}~~Under similar model sizes, among the three knowledge sources, the results revealed that the KG-based model T5-large outperformed the other methods with an average accuracy of 0.506. 

\para{HDT-QA}~~As shown in Table~\ref{tab: hdt result}, the QA-based model outperforms the NLI-based and KG-based models slightly. But overall, the performance of 3 models on the HDT-QA dataset is consistently poor. Unlike the growth in performance with increasing model size observed on the BDD-QA and TV-QA datasets, a similar trend is not as clearly visible on the HDT-QA dataset. Also, the performance of vanilla Roberta-large is comparable to that of the NLI-based and KG-based models, indicating that the contribution of NLI, and KG models to the answer to HDT-QA questions are limited. This implies that the acquisition of general knowledge is insufficient for answering questions in a human driving test. \ao{It could also imply that we need to incorporate more procedural knowledge, given the nature of the task, and that declarative knowledge is prominent in the KG resources used (well is it? I think so)} The integration of the DPR retriever, which automatically provides the most relevant paragraph, results in an improvement of 0.096 points over KG-based T5-large and 0.096 points over QA-based T5-large. This highlights the efficacy of QA models in capturing relevant domain knowledge for answering human driving test questions when complemented by a dense retrieval model that provides the most relevant evidence. The questions in the HDT-QA dataset, as exemplified in Table~\ref{tab: qaexaples}, pertain to the intricate details of driving policies and regulations. Even for human test-takers, passing the driving exam typically requires a thorough understanding of the specific rules and regulations captured in domain manuals. Therefore, incorporating domain-specific knowledge could potentially improve the ability of language models to answer these questions. On the other hand, supervised learning demonstrates high accuracy, which is expected given the overlap of knowledge between the training and test sets.



\subsection{Models' performance regarding different traffic actions in BDD-QA}
\label{bdd_rsec}

Although all three zero-shot models achieve similar overall performance, there are significant differences in their performance across different action classes. For instance, the NLI-based Roberta-large model performs well in the "Move" and "Slow" action classes, but poorly in the "Merge" and "Turn" classes. This can be explained by the nature of the actions in the "Move" and "Slow" classes, which are about following the actions of other cars, and can be easier for the NLI-based model to capture due to its strong semantic coherence capabilities. \ao{I'd imagine that the data don't contain many examples of merge and turn, being these less frequent actions than move and slow (this assumption is linked to my "granularity" comment before. This, alone, could explain the poor performance, no?}On the other hand, the KG-based Roberta-large model performs worse than the NLI-based model overall, but demonstrates better performance in the "Merge" and "Turn" classes, where semantic-level capturing is more difficult. This is due to the capability of KG-based models to capture event relations, which is inherent to knowledge graphs \ao{This would be consistent with the comment above: KG-based models are able to provide richer "semantic signals" for the representation/reasoning over merge and turn. It's not clear to me, though, why this is not observed across classes}. The QA-based T5-large model performs poorly in the "Stop" class, even below the random baseline. Further investigation is required to understand the reason for this. In general, the KG-based models show balanced performance across the 7 classes, while the NLI-based and QA-based models exhibit significant differences in performance between different action classes.

\subsection{Models' performance regarding different traffic actions in BDD-QA}


Table~\ref{tab: bdd result} shows the results for three different types of models (NLI-based, KG-based, and Multi-QA-based) on the BDD-QA dataset. 

\para{Overall performance} The T5-large model with an Information-Retrieval-Based approach yields the highest non-supervised accuracy among models with similar sizes, due to its effective knowledge extraction. However, this performance is only slightly better than the random baseline, with a difference of 0.287 points, and remains significantly behind the supervised model (0.357 points). Among the three commonly used knowledge zero-shot models (NLI, KG, QA), the KG-based models demonstrate lower performance compared to the NLI-based and QA-based models, indicating that general knowledge has a limited impact on decision-making in the traffic domain compared to semantic coherence and multi-QA training.


\para{Performance regarding different actions} Although all three zero-shot models achieve similar overall performance, there are significant differences in their performance across different action classes. For instance, the NLI-based Roberta-large model performs well in the "Move" and "Slow" action classes, but poorly in the "Merge" and "Turn" classes. This can be explained by the nature of the actions in the "Move" and "Slow" classes, which are about following the actions of other cars, and can be easier for the NLI-based model to capture due to its strong semantic coherence capabilities. \ao{I'd imagine that the data don't contain many examples of merge and turn, being these less frequent actions than move and slow (this assumption is linked to my "granularity" comment before. This, alone, could explain the poor performance, no?}On the other hand, the KG-based Roberta-large model performs worse than the NLI-based model overall, but demonstrates better performance in the "Merge" and "Turn" classes, where semantic-level capturing is more difficult. This is due to the capability of KG-based models to capture event relations, which is inherent to knowledge graphs \ao{This would be consistent with the comment above: KG-based models are able to provide richer "semantic signals" for the representation/reasoning over merge and turn. It's not clear to me, though, why this is not observed across classes}. The QA-based T5-large model performs poorly in the "Stop" class, even below the random baseline. Further investigation is required to understand the reason for this. In general, the KG-based models show balanced performance across the 7 classes, while the NLI-based and QA-based models exhibit significant differences in performance between different action classes.

\para{Effect of model size} The effect of model size on performance can be observed across different traffic actions. In general, as the model size increases, performance improves. However, the magnitude of improvement varies among action classes. For example, the "Move" class demonstrates the largest improvement, increasing from $0.468$ to $0.937$ as the model size grows. On the other hand, the "Merge" class shows a smaller improvement of only $0.068$ points. It is also worth noting that the largest Unified-QA model, T5-11B, has the same accuracy in the "Stop" class as the NLI-based Roberta-large model, despite the latter having only one-thirtieth of the parameters of the former. These results highlight the significant impact of different types of knowledge sources on performance.

\para{Result of supervised learning} The supervised training model has the highest accuracy across all action classes with scores ranging from 0.774 to 0.968. This is intuitive because the domain in BDD-QA is narrower than other typical QA models, the environment and the corresponding actions are easy to capture as a result. 



\begin{table*}[!ht]
\centering
\small
\caption{Evaluation results on the TV-QA dataset. Random baselines vary because the numbers of candidate answers vary. The human evaluation result is 1.000 because we selected the questions that are correctly answered by humans.}
\label{tab: tv result}
\begin{tabular}{c | ccccc}
\hline
\multirow{2}{*}{\bf Methods}& \multicolumn{5}{c}{\bf Reasoning Task}\\
&Event Forecasting&Reverse Reasoning& Counterfactual~~& ~~Introspective~~~~~& ~~~~~Average\\\hline
\bf Random baseline&0.353&0.299&0.438&0.468&0.373\\
\bf Roberta-large&0.323(-0.030)&0.382(+0.083)&0.384(-0.054)&\bf 0.571(+0.103)&0.412(+0.039)\\\hline
\bf MNLI-Roberta-large&0.535~(+0.182)&0.482~(+0.183)&\bf 0.589~(+0.151)&0.366~(-0.102)&0.479~(+0.106)\\
\bf CSKG-Roberta-large&0.457~(+0.104)&0.446~(+0.147)&0.358~(-0.080)&0.535~(+0.067)&0.465~(+0.092)\\
\bf CSKG-T5-large&0.577~(+0.224)&0.460~(+0.161)&0.384~(-0.054)&0.517~(+0.049)&0.506~(+0.133)\\\hline
\bf Unified-QA~large&0.485~(+0.132)&0.517~(+0.218)&0.410~(-0.028)&0.401~(-0.067)&0.468~(+0.095)\\
\bf Unified-QA~3b&0.535~(+0.182)&0.595~(+0.296)&0.435~(-0.003)&0.482~(+0.014)&0.532~(+0.159)\\
\bf Unified-QA~11b&\bf 0.718~(+0.365)&\bf 0.624~(+0.325)&0.487~(+0.049)&0.446~(-0.022)&\bf 0.597~(+0.224)\\\hline
\bf DPR+Unified-QA~large&0.464~(+0.111)&0.446~(+0.147)&0.538~(+0.100)&0.383~(-0.085)&0.444~(+0.071)\\\hline
\bf Human&1.000&1.000&1.000&1.000&1.000\\\hline
\end{tabular}
\end{table*}










\subsection{How do language models perform on traffic event analyzing and reasoning tasks? (TV-QA)}

\label{tv_rsec}

Table~\ref{tab: tv result} shows the results for three different types of models (NLI-based, KG-based, and Multi-QA-based) on the TV-QA dataset. 

\para{Effect of knowledge source} Under similar model sizes, among the three knowledge sources, the results revealed that the KG-based model T5-large outperformed the other methods with an average accuracy of 0.506. 
The NLI-based model emerged as the best performer on the \textit{Counterfactual} task with a margin of 0.1 points higher than the second-best model. Note that \textit{Counterfactual} tasks ask questions about \textit{What could happen if...}, which has a similar pattern of reasoning procedures of NLI training, this observation is intuitive. It's also worth noting that all of the models perform worse than the Vanilla-Roberta-large model, showing that the tested models are all not capable of answering questions like~\textit{What should have been done to...}.

Regarding the model size, we evaluated three variations of Unified-QA models and observed that as the model size increases, the performance improvement for surface-level reasoning tasks becomes increasingly evident. However, it's noteworthy that for the \textit{Introspective} task, the model performance actually decreases with increased model size, which is a result that deviates from typical observations of other QA tasks. Further investigation is required to understand this phenomenon.

\para{Results on different levels of reasoning tasks} Our findings indicate that zero-shot reasoning models generally perform better in the \textit{Event Forecasting} and \textit{Reverse Reasoning} tasks compared to the other two reasoning tasks. As we discussed in the task section, this can be attributed to the fact that the first two tasks can be solved through surface-level natural language understanding~e.g. \textit{what will happen next? what might happen before?}, while the latter two tasks require a deeper understanding of causal relationships and a vast amount of experience~\textit{e.g. what could happen if... or what should have been done to...}. Despite being trained on massive corpora (160GB for Roberta, 750GB for T5), the pretrained language models still demonstrate a lack of capability in capturing the cause and effect of traffic events, implying that there is room for improvement in developing knowledge-based reasoning models.



\begin{table}[!t]
	\centering
	\small
	\caption{Evaluation results on the HDT-QA dataset.}
	\label{tab: hdt result}
	\begin{tabular}{c | c}
	\hline
	    \bf Methods& \bf Accuracy\\\hline
        \bf Random baseline&0.268\\
        \bf Roberta-large&0.334\\\hline
        \bf MNLI-Roberta-large&0.324\\
        \bf CSKG-Roberta-large&0.352\\
        \bf CSKG-T5-large&0.344\\\hline
        \bf Unified-QA~large&0.414\\
        \bf Unified-QA~3b&0.432\\
        \bf Unified-QA~11b&\bf 0.456\\\hline
        \bf DPR+Unified-QA~large&0.440\\ \hline
        \bf Roberta-large(supervised)&0.822\\\hline
	\end{tabular}
\end{table}



\subsection{How do language models perform on the human driving test? (HDT-QA)}

\textbf{Result of zero-shot methods}~~As shown in Table~\ref{tab: hdt result}, the QA-based model outperforms the NLI-based and KG-based models slightly. But overall, the performance of 3 models on the HDT-QA dataset is consistently poor. Unlike the growth in performance with increasing model size observed on the BDD-QA and TV-QA datasets, a similar trend is not as clearly visible on the HDT-QA dataset. Also, the performance of vanilla Roberta-large is comparable to that of the NLI-based and KG-based models, indicating that the contribution of NLI, and KG models to the answer to HDT-QA questions are limited. This implies that the acquisition of general knowledge is insufficient for answering questions in a human driving test. \ao{It could also imply that we need to incorporate more procedural knowledge, given the nature of the task and that declarative knowledge is prominent in the KG resources used (well is it? I think so)}

\para{Retriever-based model and supervised learning} As shown in Table~\ref{tab: hdt result}, the integration of the DPR retriever, which automatically provides the most relevant paragraph, results in an improvement of 0.096 points over KG-based T5-large and 0.096 points over QA-based T5-large. This highlights the efficacy of QA models in capturing relevant domain knowledge for answering human driving test questions when complemented by a dense retrieval model that provides the most relevant evidence. The questions in the HDT-QA dataset, as exemplified in Table~\ref{tab: qaexaples}, pertain to the intricate details of driving policies and regulations. Even for human test-takers, passing the driving exam typically requires a thorough understanding of the specific rules and regulations captured in domain manuals. Therefore, incorporating domain-specific knowledge could potentially improve the ability of language models to answer these questions. On the other hand, supervised learning demonstrates high accuracy, which is expected given the overlap of knowledge between the training and test sets.


\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{figures/knowledge_fusion.pdf}\\
\caption{Granular result of transfer-learning and knowledge fusion on BDD-QA, we visualize the accuracy of 4 experiments on each action class and in average.}
\label{fig: fusion1}
\end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=\linewidth]{figures/knowledge_fusiontv.pdf}\\
% \caption{Granular result of transfer-learning and knowledge fusion on TV-QA}
% \label{fig: fusion2}
% \end{figure}


\subsection{Can traffic knowledge be transferred between different reasoning tasks?}


Figure~\ref{fig: fusion1} show the results of four models' granular performance on two datasets.

\textbf{HDT-QA dataset for transfer learning}~~In this experiment, we use the HDT-QA as a training source and assume a certain amount of traffic domain knowledge can be injected after a model training on HDT-QA. Given the multiple-choice question format of HDT-QA makes it easier for knowledge injection, we use the same training strategy as prior works did~\cite{Ma2021} on knowledge injection: given a multiple choice QA dataset, the model uses a Masked language Model to give the score of each candidate, then use the Margin Loss Function to maximize the score of the correct answer.

To assess the impact of traffic domain knowledge (HDT) on BDD-QA and TV-QA, we evaluated the HDT-QA trained model on both BDD-QA and TV-QA. We also include common knowledge from the CSKG training dataset, and fuse two training data together. Four experiments are conducted as a result: 1) vanilla Roberta-large, 2) Roberta-large trained on HDT, 3) Roberta-large trained on CSKG, and 4) Roberta-large trained on a fusion of HDT and CSKG dataset.

\textbf{Overall result} Injecting common knowledge and driving knowledge is both helpful for making correct traffic decisions, merging the knowledge leads to better performance. From figure~\ref{fig: fusion1}, the $Roberta + CSKG + HDT$ model reaches the best performance on average, followed by $Roberta + CSKG$ and $Roberta + HDT$.\footnote{The $Roberta + CK$ and $Roberta + DK$ have different sizes of training data, which is not fair to directly compare. }
The results show that combining general and driving knowledge results in better performance compared to using only one side of knowledge. The model trained with both knowledge sources indirectly transfers driving knowledge to the knowledge required for answering BDD-QA tasks, while the model trained with only driving knowledge has difficulty answering BDD-QA questions. For example, common knowledge can tell language models that cars will pass the crosswalk when driving and crosswalk will appear at the intersection, while traffic knowledge tells the models that cars should yield to pedestrians passing the crosswalk. When facing the question~\textit{what might be the reason that a car is waiting in the intersection but the traffic light is green}, the answer~\textit{The car is waiting for pedestrians} will come out, if both knowledge sources are effectively injected into the language model.

% Regarding TV-QA, injecting domain knowledge is not helpful for model performance. But again, general knowledge helps the driving knowledge be better transferred.

\subsection{Do methods' predictions agree with each other?}


The performance of a language model heavily depends on the training data and methods used. To evaluate the predictions of different models, we closely examine the results of five similarly-sized models from various knowledge sources: $Roberta-large-NLI$, $Roberta-large-KG$, $T5-large-KG$, $T5-large-QA$, $T5-large-IR$~on the BDD-QA dataset. We measure the intersection and the union of their accurate predictions, to understand their agreement and the potentially complementary results.
As shown in the left part of Figure~\ref{fig: bddoverlap}, although the models attain similar accuracy, their predictions have limited overlap with each other, with only around 50\% of their correct predictions agreeing. Even among the models $Roberta-large-KG$ and $T5-large-KG$, which have the same knowledge source, only two-thirds of their correct predictions are in agreement. This finding is consistent with the results in~\ref{bdd_rsec} and~\ref{tv_rsec} that the granular performance of different models is much more diverse than their overall performance.

The right part of Figure~\ref{fig: bddoverlap} demonstrates that the union of predictions results in significantly higher accuracy. Specifically, combining the $Roberta-large-NLI$ and $T5-large-IR$ models results in an accuracy of $0.757$, with a gap of only $0.137$ compared to supervised learning methods. These results are much higher than the performance of each model individually and are close to the results obtained from supervised learning. These findings motivate the need for the development of methods that combine model predictions in a fine-grained manner.


\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{figures/bdd_overlap.pdf}\\
\caption{A heat map representing the intersection(overlap) and union of correct predictions on BDD-QA for five models of similar size(large models). Each value in the heat map represents the proportion of the intersection/union of correct predictions of two models to the total data, i.e., the accuracy of the intersection/union.}
\label{fig: bddoverlap}
\end{figure}


\subsection{Case study}


In section~\ref{bdd_rsec}, we have observed in BDD-QA NLI-based models are more likely to choose the actions that follow other cars', while KG-based models can capture more abundant relations due to the structure of the knowledge graph. To further justify this hypothesis, we use two examples of traffic-domain decision-making questions and show two models' prediction distributions. From the first plot of~\ref{fig: case}, given the question \textit{Traffic ahead of the car is beginning to move, what does the car do next?}, NLI-based model chooses the correct answer \textit{The car is advancing slowly.} while the knowledge model chooses the wrong answer \textit{The car reduces its speed}. As we discussed, the NLI-based model wins this question by capturing the semantic coherence between \textit{move} and \textit{advance}. For the second plot of~\ref{fig: case}, given the question \textit{The car wants to move into another road, what does the car do next?}, the NLI-model still chooses the answer based on semantic similarity without noticing the car is moving to another road. While the KG-based model makes the correct choice by successfully connecting the car action \textit{turn} with the description \textit{move into another road}

\begin{figure}[!t] 
\centering
\includegraphics[width=\linewidth]{figures/case.pdf}\\
\caption{Two models' prediction distributions of two typical traffic decision-making questions. Questions are computed on the top of each plot, and candidate answers are presented at the bottom. The probabilities are given by the scores of each answer outputted by the model through a soft-max layer.}
\label{fig: case}
\end{figure}
